Multi-Step Recurrent Q-Learning for Robotic Velcro Peeling

Learning object manipulation is a critical skill for robots to interact with their environment. Even though there has been significant progress in robotic manipulation of rigid objects, interacting with non-rigid objects remains challenging for robots. In this work, we introduce velcro peeling as a representative application for robotic manipulation of non-rigid objects in complex environments. We present a method of learning force-based manipulation from noisy and incomplete sensor inputs in partially observable environments by modeling long term dependencies between measurements with a multi-step deep recurrent network. We present experiments on a real robot to show the necessity of modeling these long term dependencies and validate our approach in simulation and robot experiments. Our results show that using tactile input enables the robot to overcome geometric uncertainties present in the environment with high fidelity in ~90% of all cases, outperforming the baselines by a large margin.

==> mujoco_fig.tex <==
\begin{figure}[t!]
	
	\centering
	\begin{subfigure}{0.43\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/velcro_parameters.png}\caption{Velcro parameters}\label{fig:velcro_param}
	\end{subfigure}
	\vskip\baselineskip
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/cylinder_velcro.png}\caption{Cylinder velcro}\label{fig:velcro_model}
	\end{subfigure} \hfil
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/sim_env.png}\caption{Simulation setup}\label{fig:sim_env}
	\end{subfigure}
	\caption{(\ref{fig:velcro_model}) The velcro strip model in simulation: point masses (grey spheres) connected by stiff spring (grey cylinders), attached by hook and loop tendons (green cylinders). (\ref{fig:sim_env}) Robot agent setup which consists of a parallel jaw gripper and a velcro strip with a handle to grasp. }
	\label{fig:mujoco}
\end{figure}

==> network.tex <==
\begin{algorithm}[htpb!]
    \caption{Multi-step DRQN Learning with tactile feedback}
    \label{alg:drqn}
    \SetAlgoLined
    Initialize replay memory $D$ with capacity $N$, tactile sequence networks $Z_{\omega}$ and Q-networks $Q_{\theta1}$, $Q_{\theta2}$ \\
    $i \leftarrow 0$\\
    \While{$i <$ \text{max iterations}}
    {
        $t=0$\\
        $h_0 \leftarrow 0$ LSTM hidden state\\
        $o_t \leftarrow \mathcal{O}(s_t)$ observe tactile measurement \\
        \While{$o_t \neq $ \text{terminal}}
        {
            With prob. $\epsilon$ select random action, otherwise $a_t, h_t = \text{argmax}_a^*Q(z, h_{t-1}|\theta_i)$\\
            \While{$o_t$ \text{contains weak tactile feedback}}{
                Take action $a_t$\\
                Get next observation and reward $(o_{t+1}, r_t)$
            }
        Update hidden vector $z = Z_{\omega}(o_t, ..., o_{t+k})$   \\
        Store transition $\{o_t, ..., o_{t+k}\}, a_t, r_t$ in $D$\\
        $t \leftarrow t + k$
        }
    }
    \For{\text{each update step}}
    {
        Sample transitions of tactile sequence from $D$\\
        \For{\text{sequence} $(seq_{j}, a_j, r_j, seq_{j+1})\text{ in batch}$}
        {
            Compute tactile hidden vector $z_i = Z(seq_j|\omega)$  \\
            $h_{j-1} \leftarrow 0$ \\
            \For{$k=j$ to $k=j+\tau$}{
                Update hidden state $h_k = Q(z_k, h_{k-1}|\theta_i)$
            }
            Compute target Q value: 
            $Q^*(z_j, a_j) = r_j + \gamma \max_{a*}Q_{\theta i}(z'_{j}, a', h_{j+\tau)} | \theta_i)$ \\
            Optimize parameters $\theta, \omega$ with loss:  $|Q^*(z_j, a_j) - Q_{\theta i}(z_{j}, a_{j})|_1$
        }
    }
\end{algorithm}


